The ASTRID simulation: the evolution of Supermassive Black Holes

We present the evolution of black holes (BHs) and their relationship with their host galaxies in Astrid, a large-volume cosmological hydrodynamical simulation with box size 250 $h^{-1} \rm Mpc$ containing $2\times5500^3$ particles evolved to z=3. Astrid statistically models BH gas accretion and AGN feedback to their environments, applies a power-law distribution for BH seed mass $M_{\rm sd}$, uses a dynamical friction model for BH dynamics and executes a physical treatment of BH mergers. The BH population is broadly consistent with empirical constraints on the BH mass function, the bright end of the luminosity functions, and the time evolution of BH mass and accretion rate density. The BH mass and accretion exhibit a tight correlation with host stellar mass and star formation rate. We trace BHs seeded before z>10 down to z=3, finding that BHs carry virtually no imprint of the initial $M_{\rm sd}$ except those with the smallest $M_{\rm sd}$, where less than 50\% of them have doubled in mass. Gas accretion is the dominant channel for BH growth compared to BH mergers. With dynamical friction, Astrid predicts a significant delay for BH mergers after the first encounter of a BH pair, with a typical elapse time of about 200 Myrs. There are in total $4.5 \times 10^5$ BH mergers in Astrid at z>3, $\sim 10^3$ of which have X-ray detectable EM counterparts: a bright kpc scale dual AGN with $L_X>10^{43}$ erg/s. BHs with $M_{\rm BH} \sim 10^{7-8} M_{\odot}$ experience the most frequent mergers. Galaxies that host BH mergers are unbiased tracers of the overall $M_{\rm BH} - M_{*}$ relation. Massive ($>10^{11} M_{\odot}$) galaxies have a high occupation number (>10) of BHs, and hence host the majority of BH mergers.

==> trash.tex <==

% Michael Tremmel: similar to before, I think a reminder to the reader as to the differences in your NH and what is being probed with AGN observations. Your values are really lower limits right, given that gas on much smaller scales could be dominating but remains unresolved?
% Michael Tremmel: Still, given that you match the observations pretty well, that is additional evidence that the majority of obscuring gas is coming from the galaxy and not the torus? Worth mentioning here again maybe?

% However, $N_{\rm H}$ see along AGN lines of sight is mainly contributed by the innermost regions of galaxies (< 10 ckpc/h) and is subject to large variation due to AGN feedback. $N_{\rm H}$ therefore does not exhibit a tight power law relation with the $M_*$, because of the large angular variations present in the massive systems.
% The above two observations probe $N_{\rm H}$ through AGN lines of sight. 
% Additionally, \cite{Buchner2017} probe galactic obscuration through $N_{\rm H}$ values inferred from the X-ray spectra of GRBs, and study how $N_{\rm H}$ varies with respect to GRB host galaxy mass. These authors find that $N_{\rm H} \propto M_*^{0.38}$ in the redshift range $1<z<5$, implying that galactic obscuration scales with the galaxy size.
% We note here, however that $N_{\rm H}$ see along AGN lines of sight is mainly contributed by the innermost regions of galaxies (< 10 ckpc/h) and is subject to large variation due to  AGN feedback. $N_{\rm H}$ therefore does not exhibit a tight power law relation with the $M_*$, because of the large angular variations present in the massive systems.
% The red and grey error bars show HSC observations of $z>6$ quasars from \citet{Izumi2021}.



% Compared with TNG-300 where the BH population steeply spikes at the seed mass of $10^6 \hmsun$, BHs in \asterix extends down to lower seed mass with a flatter slope due to the power-law seeding.
% At the more massive end, we extend to slightly larger BH mass range compared with TNG-300 with a larger volume.
% At $z=4$, the BH population at $\mbh > 10^7 \msun$ is in good agreement with the prediction from \cite{Ueda2014} inferred from X-ray observations.
% as the volume of \asterix is about 1.7 times larger compared to TNG-300. 
% We note that the BH number densities at the small mass end are sensitive to the seeding prescriptions and on the initial growth before reaching the phase of self-regulation modulated by AGN feedback.
% with a generally smaller seeding mass it marginally miss the population of the first $10^9 \msun$ QSOs at $z>6$ regime which are thought to power the high-$z$ quasars
% \yueying{Do we want to add BlueTides for comparison?}




% For example, \cite{Volonteri2016Horizon-AGN} suggested that the overprediction of faint-end AGN could be due to inefficient supernovae feedback (i.e. the removal of gas in the galaxy responsible for both nuclear accretion and star formation as a consequence of supernovae activity) being underestimated in low-mass haloes in simulations and bring higher accretion to the BHs residing there.

% This discrepancy suggests that the modelling of the small-mass BHs need to be improved.
% As seen in Figure~\ref{fig:BH-XLF}, 
% Therefore, exclusion of small mass BHs or BHs residing in the small halos can also play a role at the faint end \citep[e.g. ][applied $\mbh < 5 \times 10^7 \msun$]{Sijacki2015}.

% The $L_{\rm BH} - \mbh$ relation is steep at low mass end where BH growth is dominated by the initial Bondi-Hoyle-Lyttleton-like accretion, with more massive BHs enduring higher accretion rate, and on average gives higher Eddington accretion ratio $\lambda_{\rm Edd} \equiv \dot{M}/\dot{M}_{\rm Edd}$ when $\mbh \lsim 10^7 \msun$. 
% and keep approaching the upper limit corresponding to the Eddington accretion (marked as the gray dotted line).
% At the more massive regime, the $L_{\rm BH}-\mbh$ curve starts to bend over when approaching the massive end.
% As shown by the background $L_{\rm BH}-\mbh$ distribution at $z=3$, some BHs in mass regime of $\mbh < 10^7$ can still approach the upper limit of $L_{\rm Edd}$, while more massive BHs with $\mbh > 10^7 \msun$ can hardly reach $L_{\rm Edd}$, as the AGN feedback starts to take effect and self-regulate the BH growth.
% Massive BHs dump thermal energy to the surrounding and the resultant hot sparse gas slow down the BH accretion.
% As a result, the Eddington accretion ratio $\lambda_{\rm Edd} \equiv \dot{M}/\dot{M}_{\rm Edd}$ is far from being saturated for massive BHs. 
% so close to the maximum allowed value, given they come from a distribution of seeds that should span that whole range? Is it because at this mass the final mass is more or less tracking the initial mass so a 1e6 BH must have come from a pretty massive seed?


% It has now been well established from X-ray studies that the vast majority of AGN are obscured by thick columns of gas and dust.
% Traditionally, AGN obscuration is associated with the “torus”, a nuclear structure (on scales of $\sim 10$ pc) surrounding the accretion disk on the BH. 
% However, it is still very much debated how much of the obscuration could also take place by the galactic gas, particularly at high redshift.
% In the simulation, we can directly assess the contribution to the obscuration due to the gas in the host galaxy \citep[mostly due to the same, cold gas reservoir is responsible for fuelling the AGN; See][]{Ni2020}.
% In Figure~\ref{fig:BH-XLF}, we show in the dashed-dotted line the AGN population with $\NH>10^{23} \mathrm{cm}^{-2}$, with the $\NH$ threshold following the convention of \cite{Vito2018}.
% Note that $\NH$ calculated here is the galactic obscuration as the lower limit of the total obscuration, as we can not resolve the nuclear scale "torus".


% In Figure~\ref{fig:BH-XLF} we also show the predictions for the {\it obscured} AGN population (inferred by calculating the contribution to $\NH$, due to galactic scale gas component, see next Section) and for the BH population with $\mbh > 10^{7} \msun$. 
% Here we define obscured AGN as $\NH>10^{23} \mathrm{cm}^{-2}$ following the convention of \cite{Vito2018}.
% The derived XLFs are similar at the bright end (for luminosities $\log \Lx > 43.5$) while they differ at faint end. 
% In both cases, whether we look at the obscured AGN or those with BH mass larger than 
% However, we also note that the predictions of the XLF, particularly at the faint end, are sensitive to the amount of obscuration to the AGN. 
% It has now been well established from X-ray studies that the vast majority of AGN are obscured by thick columns of gas and dust.

% Estimating the contribution of the elusive Compton thick AGN remains challenging and cause implete
% As the faint end is dominated by small mass BHs that not yet reached the self-regulated regime, 
% \asterix show good 
% The left and middle panel of Figure~\ref{fig:BH-XLF-UVLF} give the X-ray luminosity function at $z = 7 \sim 6$ and $z = 5 \sim 4$ respectively, with observational predictions collected from \cite{Ueda2014,Aird2015,Buchner2015,Vito2018}. 
% Compared with X-ray observations, \asterix simulation predicts a steeper slope at the fainter end. 
% However, we also note that the faint AGN is subject to the gas obscuration of their host environment and is therefore challenging to detect for X-ray observations ..

% Our main result is that the host galaxy gas provides a luminosity-dependent obscurer (a positive correlation), for which we compute covering fractions. 
% \tiziana{In principle Ueda et al. 14 provide some observationally inferred fits to account for the NH 'suppression' - we could use these fits to estimate the effect at the faint end
% (these were also used by the recent paper by Yuang et al. 21 (SAMs) and also in Shen et al 2020 bolometric LFs}
% \tiziana{please add something about the covering fraction as a function of NH plot- I am really not sure what this plot shows...it seems to me that these are consistent with what expected/gray area? }

% As indicated in the legend, the red to orange coloured lines in the left panel split the BHMD by different BH mass range, and the purple to blue coloured lines in the right panel show the BHAD contributed by BHs from different luminosity range.
% \textcolor{red}{Usually in papers the figure captions aren't repeated in the text - the text is to give insight into what the figures are about. I guess it's too late for this paper but really the captions should have less detail (for example about the assumptions made by the observers whose points are being plotted) - those details should be in the text, along with inferences made from the plots.}

% Michael Tremmel: It would be nice to mention previous results related to this. Ricarte+ 2019 showed in Romulus a roughly constant relationship between SFR and BHAR for galaxies . Mulaney+ 2012 had observational predictions related to this as well.

% The upper limit does not include Compton-thick AGNs
% The gray shaded area 
% In this section, we show the global statistics of the BH growth in \asterix.
% The left panel of Figure~\ref{fig:BHrate-history} gives the evolution of the BH mass density (BHMD) from $z=11$ to $z=4$.
% Current upper limits from X-ray observations are presented in triangles, from \cite{Salvaterra2012} [cosmic X-ray background (XRB)] and \cite{Treister2013}.
% As comparison, we also give predictions from \cite{Volonteri2016} (purple shade) inferred from the scaling relation with the host galaxy mass.
% The right panel of Figure~\ref{fig:BHrate-history} gives the BH accretion rate density predicted by Asterix...

% \tiziana{this is still v. confusing... I thought compared to all BHs / mass function}.
% The dashed lines include only $M_1$ so that it presents the averaged rate for BHs swallow another smaller mass BH.
% \textit{Third panel}: The averaged merger rate for BHs from a given $\mbh$ bin. Orange, green and blue lines show results at redshifts $z=5$, $z=4$ and $z=3$ respectively. The solid lines include both $M_1$ and $M_2$ when counting BH mergers. The dashed lines include only $M_1$ so that it presents the averaged rate for BHs swallow another smaller mass BH. The dashed-dotted lines include  $M_1$ and $M_2$ for the non-seed BH merger events where both BHs have $\mbh > 2\times \msd$ at the moment of merger.
% \yueying{middle panel plot add dual component?}
% Michael Tremmel: I find this figure confusing... would it just be easier to plot three different bins in mass ratio? any, q > 0.1 and q < 0.1 or something? Also, how can the MBH > 2 Mseed be so much lower at Mbh ~ 1e8? The dashed+solid lines seem to indicate that most of these mergers have both M1 and M2 of similar mass, which is already much larger than 2 Mseed. Or am I misinterpreting something here?


% Remind that the distance criteria for BH merger $|\bf{\Delta r}|$ $< 3 \hkpc$ implies that the binary BHs are embedded in similar gas environment at the time of merger, therefore both BHs are likely to have the same order of luminosity if their $\mbh$ is in the same order.
% \yueying{Comment on the mean mass of the pairs are visible/dual AGN}
% \yueying{Comment on the number of occupation number>1 for Lx>43}
% \yueying{A bit weird to put here, maybe more comments why it is interesting. AGN duals.}
% \colin{Maybe slightly clarify the condition for the brown line.  Is the condition that there must be a moment in time when both BH1 and BH2 simultaneously have $L > 10^{43}$, or that each of the BHs must have had $L > 10^{43}$ during the separation, but not necessarily simultaneously?  I assume it's the latter, to make it consistent with the ability to observe a dual AGN, but it would be good to state it explicitly.}


% This trend is mainly due to the fact that massive galaxies, which are the hosts of the most massive BHs, have a large BH occupation number, as shown in Figure~\ref{fig:Occupation}.
% More massive BHs residing in larger galaxies are more likely to encounter other BHs from the other subgroups, 
% while low mass BHs residing in more isolated galaxies have fewer chances to merge.

% lower panel would suggest a z=5 BH with M∼106.5Mwouldbe expected to undergo about 1 merger per Gy
% The $y$ axis is in unit of merger rate per comoving volume at a given redshift $z$, obtained by averaging the merger rate calculated in a 300 Myr bin centered at $z$, over the BHs in each $\mbh$ bin at that time $z$.
% The solid lines include both $M_1$ and $M_2$ when counting BH mergers, giving the averaged merger rate for BHs from a given $\mbh$ bin to merge with any other BHs.
% The dashed lines include only $M_1$ for each BH merger. They give the rate for BHs to swallow another smaller mass BH and therefore is much lower at the small $\mbh$ end compared with the solid lines.
% Finally the dashed-dotted lines count only the non-seed mass mergers where both BHs have $\mbh > 2 \times \msd$ at merger time, with both $M_1$ and $M_2$ included. 
% The dashed-dotted lines drop off at $\mbh < 10^6 \msun$, as most of the BHs there are in the seed mass regime.


% Also, as established from the analytical estimates \citep[e.g.][]{Binney2008}: the dynamical friction time is proportional to the velocity dispersion of the primary galaxy, and is in turn positively correlated with the mass of the primary BH;
% Moreover, $\mbh$ also plays crucial role in dynamic friction. As established in \cite{Chen2021}, more massive BHs embedded in large galaxies (with high density of collisionless particles) would undergo larger dynamic friction that dissipate the kinetic energy more rapidly, as a result they will sink to galaxy centers in a shorter time scale and merge with other BHs.

% There are about $1.5 \times 10^5$ BH mergers in Asterix at $z>4$. 
% The first panel of Figure~\ref{fig:BH-merger-history} gives the BH merger rate history as a function of the redshift.
% The black line includes all the BH mergers. 
% The orange line show the merger rates for BHs that go beyond the seed mass, including mergers with the criteria $M_2 > 5 \times 10^5 M_{\odot}$.
% The red line include the mergers with a higher mass ratio with $M_2/M_1 > 0.3$.
% The right two panels of Figure~\ref{fig:BH-merger-history} show the distribution of BH mass (second panel) and ratio (third panel) for all the merger events.
% We can see that BH mergers are mostly contributed by events involving the small seed mass BHs. On the other side, the distribution of the BH mass ratio $q \equiv M_2/M_1$ is close to uniform in the range of $q \sim$ [0, 1]. 

% To quote a number, there are 3200 mergers with one BH having luminosity $\log \Lx > 43$ at the time of merger. Apart from that, we also look for bright dual AGNs with $\log \Lx > 43$ that could be observed by Lynx. 
% We trace the BH trajectories for the merger populations and find that there are 115 BH mergers with both $\log \Lx > 43$ at the separation [5,10] $\hkpc$ before they merge.

